Graph-based Cluttered Scene Generation and Interactive Exploration using Deep Reinforcement Learning

We introduce a novel method to teach a robotic agent to interactively explore cluttered yet structured scenes, such as kitchen pantries and grocery shelves, by leveraging the physical plausibility of the scene. We propose a novel learning framework to train an effective scene exploration policy to discover hidden objects with minimal interactions. First, we define a novel scene grammar to represent structured clutter. Then we train a Graph Neural Network (GNN) based Scene Generation agent using deep reinforcement learning (deep RL), to manipulate this Scene Grammar to create a diverse set of stable scenes, each containing multiple hidden objects. Given such cluttered scenes, we then train a Scene Exploration agent, using deep RL, to uncover hidden objects by interactively rearranging the scene. We show that our learned agents hide and discover significantly more objects than the baselines. We present quantitative results that prove the generalization capabilities of our agents. We also demonstrate sim-to-real transfer by successfully deploying the learned policy on a real UR10 robot to explore real-world cluttered scenes. The supplemental video can be found at https://www.youtube.com/watch?v=T2Jo7wwaXss.

==> Related_work.tex <==
Our work falls within the broad domain of interactive perception~\cite{bohg2017interactive}, which involves leveraging interaction to infer otherwise hidden properties about an environment, such as masses of objects~\cite{xu2019densephysnet,kumar2019estimating}, state of a cluttered scene~\cite{novkovic2020object,poon2019probabilistic} or kinematic structure of articulated objects~\cite{katz2011interactive}.
% We break down the prior work into three categories: object search, scene generation, and object rearrangement.
% More specifically, our work share common ground with object search, scene generation and object rearrangement, which we discuss in the following subsections.
\paragraph*{Object Search in Robotics}
Building robots that can help in domestic households has been a long-standing goal of robotics. It is important for such robots to be able to search and retrieve objects in cluttered scenes. This involves first finding an object, singulating it, planning a grasp, and then actually executing motor commands. Let us assume that modern CNN-based approaches are powerful enough to find objects despite significant occlusions. But even when all objects are completely visible, grasping can be quite challenging if many objects are in close proximity. Therefore, a body of work in object singulation focuses on moving objects in clutter such that they are spread out and do not touch each other \cite{sarantopoulos2019split,chang2012interactive,eitel2017learning}. Once the objects are singulated, planning of feasible grasps becomes much easier as grasping does not depend on the clutter surrounding it. 

There also exist other approaches that deal with occluded objects that may be partially or completely invisible~\cite{kurenkov2020visuomotor, danielczuk2019mechanical, zeng2018learning, deng2019deep, yang2020deep}. Often in such heavily cluttered scenes, the agent has to move other objects around to search for the target. Prior works have investigated common environments, such as a bin~\cite{danielczuk2020x,kurenkov2020visuomotor,novkovic2020object,danielczuk2019mechanical} or a shelf~\cite{li2016act,huang2020mechanical}.
While learning to retrieve a target object from a collection of objects thrown randomly into a bin is useful in some scenarios such as warehouses, structured clutter is more common in spaces with where humans interact, like kitchen pantries or supermarket shelves. Arranging objects with some underlying structure helps us recollect where each object is located, aiding in quick retrieval. Additionally, it also ensures that the objects themselves do not get damaged due to large localized contact forces, frequently encountered within object piles in bins.
% Another distinction that has been made by prior work is on the nature of clutter itself rather than its location. Objects can either be randomly dropped into a bin\cite{danielczuk2020x,kurenkov2020visuomotor,novkovic2020object,danielczuk2019mechanical} or can be arranged following some underlying structure\cite{murali20206,sui2017goal,sui2020geofusion}. % repeated?
% , like how objects are arranged in a kitchen pantry where objects are stacked on beside and on top of each other creating structured clutter, inherently favouring some arrangements over others. In \cite{murali20206} the authors investigate grasping strategies to retrieve target objects from such structured clutter. \sehoon{maybe this can be merged to the scene generation section.}

While these approaches learn to search for a given target object, a more generalized version of this problem is to identify and locate \textit{all} objects present in the scene. Estimating the \emph{state} of such structured cluttered scenes has been explored by prior works~\cite{sui2017goal,sui2020geofusion} by using passive and active perception techniques.
Another approach to tackle the problem as investigated in~\cite{poon2019probabilistic} is to get the scene to a state where all objects in the scene are clearly visible. However, this may not always be feasible as the robot might have to operate in environments where extra space might not be available. Their approach also relies on a priori knowledge of the number of objects in the scene. % or for objects more complex than simple cuboids. 
Similar to~\cite{poon2019probabilistic}, our objective is also to estimate the underlying true state of the scene. However, we take a reinforcement learning based approach to understand scenes by rearranging objects in a confined bin, that can generalize to scenes with arbitrary number of objects. 
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{images/overview_v3.png}
\label{fig:architecture}
\caption{Overview of our method. We train two agents with conflicting objectives while ensuring that the scene remains stable. The Scene Generation agent (SG) tries to hide more objects in the scene while the scene exploration agent (SE) tries to find them. Each MP-step consists of a message passing layer followed by Global Attention~\cite{li2015gated} with a skip connection.}
% \sehoon{This is good. Can you add captions to the graph (with circles). People will not know it without reading figures.}}
\end{figure*}
\paragraph*{Scene Generation}
Synthetic scene generation is an important area of research that has applications in computer vision, robotics and computer graphics. The goal is to create synthetic counterparts of realistic scenes that share resemblance at a structural and semantic level. A natural choice of representation for scenes is a scene graph, which typically represents objects as nodes and uses the edges to represent relational attributes between objects~\cite{krishna2017visual,liu2014creating, wang2019planit}. A body of work in scene generation~\cite{zhou2019scenegraphnet,devaranjan2020meta,qi2018human} focuses on creating 3D scenes by first creating scene graphs and then instantiating the represented scene using a renderer. 
Such a representation is used by \cite{zhou2019scenegraphnet} to determine which object can be added to an existing scene while satisfying the semantic narrative. This requires the construction of a graph by sequentially adding specific nodes and edges at specific locations on an intermediate graph.
% , such that it fits into the semantic narrative of the room (for example a television is more likely to be in a living room than a bathroom). Other approaches construct entire scenes instead of just augmenting an already existing synthetic scene. This requires the construction of a graph by sequentially adding specific nodes and edges at specific locations on an intermediate graph. \sehoon{Maybe we can cut a few sentences, because it is not about robotics.}


Formal systems \cite{chomsky2009syntactic} offer a promising alternative approach. 
A formal system is defined by a set of non-terminal nodes, terminal nodes and production rules that define transformation from one sequence to another.
These systems were originally formulated to tackle natural language processing and linguistic problems, but can be modified to represent graphical structures.
Production rules can then be defined to add, remove or change nodes and edges in the graph. In \cite{lau2011converting}, the authors define such a formal system to disintegrate furniture models and represent them using primitive shapes. More recently, ~\cite{devaranjan2020meta,purkait2020sg} utilized a stochastic scene grammar to generate simulated scenes that mimiced the structure and semantics of a real-world dataset. In contrast, we take a self-supervised approach to scene generation that is grounded in physical plausibility, by building scenes with cluttered but stable object arrangements in a \textit{physics simulator}.
%%SH: I deleted the below since it is a bit out of context
% Scene grammar has also been explored in the robotics research community to learn skeletal structures that can effectively navigate difficult terrain \cite{Zhao2020robogrammar}. 
% They use a recursive graph grammar that is optimized by a reinforcement learning agent to generate a skeleton that can traverse the terrain efficiently. In our problem we use a similar recursive grammar to define our scenes but we want our scene generator to create a distribution of adversarial scenes instead of just one scene containing hidden objects.
In the work of \cite{sui2017goal}, scene graphs are used along with a particle filter to represent multiple hypothesis of  the underlying object-object relationships in the scene. They however assume that all the objects in the scene are visible and identifiable.  In our case, the scenes frequently contain heavily occluded objects that even a state-of-the-art object detector will not be able to identify. Instead, we take an RL based approach and learn manipulation strategies that can efficiently uncover these objects.

% \vspace{-2mm}
\paragraph*{Object Rearrangement}
Object rearrangement in the context of robotic manipulation has been investigated by prior works \cite{batra2020rearrangement,zeng2020transporter,danielczuk2020object}. In a typical object rearrangement scenario, the agent is given a goal state (either explicit or implicit, such as organizing a pile of grocery items in a pantry). Similarly, in our work we train the agent to rearrange objects in the scene with the objective of revealing hidden objects. However, in contrast to prior approaches in object search~\cite{danielczuk2020x,danielczuk2019mechanical}, we \emph{do not require an auxiliary bin} to discard occluding objects. This provides our robotic agent two advantages: \emph{(i)} In real world environments, the robot may not have access to an additional space where it can discard objects, giving our approach a competitive edge; and, \emph{(ii)} At the end of its sequence of interaction, our robot knows the location and identity of every object present in the scene and can be asked to retrieve multiple objects without any additional exploration. 
% This makes our work appropriate for real world tasks that might require adapting to continuously varying goals.
% While we do not have a singular goal state in our problem, we have distribution of states, which when reached give the robot a complete understanding of the scene.
% Instead, our goal is to completely understand the given scene, via object rearrangement with multiple interactions.
% While rearranging objects our robot executes controlled manipulations that moves the state of the scene through a series of partially observed states that gradually pull together the robot's belief about the world and the true underlying state.



==> architecture.tex <==
\subsection{Architecture}
Scene graphs form the backbone of our approach. Hence, to build our agents we use Message Passing Neural Networks (MPNNs) that can extract high level features from graphs by propagating messages between nodes. 
In what follows, we discuss the scene graph representations that we use as input, and the model architecture of our agents as well as the object detector. %below:

\textbf{Scene Generation Agent:} For the scene generation agent we represent the nodes of the scene graph as the concatenation of a one-hot vector encoding the node type, a boolean flag \textit{is\_simulated} that represents if the node has been simulated, and the $3$ dimensional position of the node if \textit{is\_simulated} is set to be True. The edges of the scene graph are represented as one-hot vectors that specify the type of the edge. Before feeding the scene graphs into a network, we first embed each node using a fully connected (FC) layer followed by a non-linearity (Leaky-ReLU), resulting in a vector of  $32$ dimensions. We use a similar network to embed the edges into a vector of size $3$. 
The network architecture is similar to the one used by \cite{janisch2020symbolic} for BlockWorld. 
Consider an input scene graph G consisting of nodes from $\mathcal{V}$ and edges from $\mathcal{E}$. A Message Passing Neural Network is defined by a message aggregating function $\phi_{agg}$ that aggregates incoming messages from all the neighbours of a node, an update function $\phi_{update}$ that updates the features of a given node based on the received messages and a message embedding function $\phi_{msg}$ that creates a message from a sender node $e.s$ to a receiver node $e.r$ over an edge $e$. In our experiments, we aggregate messages as follows: 
\begin{equation}
\forall v: m_{v}=\max _{e . r=v} \phi_{m s g}(e, e . s)
\label{eq:aggr_function}
\end{equation}
The aggregated messages are then used to update the node features:
\begin{equation}
\forall v: v^{\prime}=v+\phi_{a g g}\left(v, m_{v}, g\right)
\label{eq:update_function}
\end{equation}
Here $g$ represents a global node that embodies features from the entire graph using a Global Attention~\cite{li2015gated} Layer and a skip connection, defined as follows:
\begin{equation}
\left.g^{\prime}=g+\phi_{g l b}\left(g, \sum_{v \in \mathcal{V}} \phi_{a t t}(v) \cdot \phi_{\text {feat }}(v)\right)\right)
\label{eq:global_node}
\end{equation}
$\phi_{att}$ is a single liner layer followed by a softmax and $\phi_{feat}$ and $\phi_{glb}$ are single linear layers followed by a Leaky-ReLU. The above steps, equations \ref{eq:aggr_function}, \ref{eq:update_function}, \ref{eq:global_node}, denote one step of our Multi-Message Passing architecture. In our experiments, we repeat this step $4$ times and pass $g^{\prime}$ from the last step through a linear layer to generate the Q-values for all the rules in our graph grammar. See table \ref{tab:hyperparameters_scene_generation}, for details about hyper parameters.
% \deleted{ We train this agent with Soft Q-Learning for a total of $64k$ steps starting with a learning rate of $5\times 10^{-5}$ and halving it every $2k$ steps. The network architecture is similar to} \cite{janisch2020symbolic} \deleted{albeit we utilize $4$ message passing layers. We pass the output of the GlobalAttention layer through a FC layer to generate Q-values for all the rules in our graph grammar. We train the agent for a total of $64k$ steps starting with a learning rate of $5\times 10^{-5}$ and halving it every $2k$ steps.}
% Our network consists of $4$ message passing layers each of which has an FC layer that appends the node and edge features to create $32$ dimensional vector. We also use a Global Attention layer that consolidates from all nodes of the graph at each stage and passes it to the next stage. The aggregating function of each layer concatenates the node features with the global attention output and 

\textbf{Scene Exploration Agent:} It uses a similar scene graph representation with a few modifications. For the Privileged Agent, it uses an \textit{is\_seen} flag instead of an \textit{is\_simulated} flag to indicate whether an object has been seen or not. The node features also contain the orientation of the object represented as quaternions. The edges of this graph are represented with a single boolean flag to denote if the two objects are connected. 

    We use architecture identical to \cite{janisch2020symbolic} to compute the value of the state and actions. 
The privileged Scene Exploration agent computes the value of a state and a probability distribution over pick and place nodes as output. The value is computed by passing $g^{\prime}$ from the final Global Attention layer through a linear layer that outputs a single value for a given input state. To compute the probability distribution over nodes, the node features are passed through a linear layer that outputs a single value, which is then mapped to a probability distribution using a softmax function.
The same architecture is utilized for the Student Agent, but we drop the FC network that computes the value function as we directly maximize the log probabilities of the actions through Behavior Cloning from expert trajectories generated by the privileged Exploration Agent.

\textbf{Object detector:} We utilize the Scaled-YOLOv4 \cite{wang2020scaled} network as the object detector. First, we create simulated scenes by dropping $20$ objects (randomly sampled from the set of objects defined previously) into a bin and collect a dataset of 100k images. We then augment this dataset with 10k images of scenes generated by a random scene generation agent. In each case, we capture an image from the overhead RGBD camera and record the bounding box annotations for all objects in the scene. This data collection pipeline ensures that we include a significant proportion of partially and completely occluded objects in our dataset. We train the network on this dataset and use it as the object detector throughout our paper.
% \vspace{-50pt}

==> backup.tex <==
Separate tables
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{Num. Nodes} & \multicolumn{2}{c|}{Objects Hidden} & %
    \multicolumn{2}{c|}{Stability Index}\\
\cline{2-5}
%  & \multicolumn{2}{c|}{Value} & \multicolumn{2}{c|}{Value} & \\
% \cline{2-5}
 & RU Agent & SG Agent & RU Agent & SG Agent \\
\hline
10 & 0.9492 & \textbf{2.0988} & 0.84 & \textbf{0.99} \\
% 11 & 0.9559 & \textbf{2.3655} & 0.79 & \textbf{0.95} \\
% 12 & 0.904 & \textbf{2.3618} & 0.8 & \textbf{0.98} \\
% 13 & 1.1544 & \textbf{2.2795} & 0.78 & \textbf{0.97} \\
% 14 & 0.9792 & \textbf{2.328} & 0.64 & \textbf{0.97} \\
15$^*$ & 1.0496 & \textbf{2.3859} & 0.64 & \textbf{0.99} \\
% 16 & 1.0595 & \textbf{2.3232} & 0.65 & \textbf{0.96} \\
% 17 & 1.2474 & \textbf{2.2932} & 0.63 & \textbf{0.98} \\
% 18 & 1.27968 & \textbf{2.2736} & 0.62 & \textbf{0.98} \\
% 19 & 1.0556 & \textbf{2.1945} & 0.52 & \textbf{0.95} \\
20 & 1.199 & \textbf{2.2878} & 0.55 & \textbf{0.93} \\
25 & 1.0291 & \textbf{2.4381} & 0.41 & \textbf{0.81} \\
\hline
% \label{tab:scene_generator_results}
\end{tabular}
 \caption{\label{tab:scene_generator_results} Performance of the Scene Generator Agent (SG) compared to Random Uniform Agent (RU). Stability index is the fraction of simulated scenes that end up being physically stable.}
\end{table}
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{Num. Nodes} & \multicolumn{2}{c|}{Fraction of scenes solved} & %
    \multicolumn{2}{c|}{Objects found}\\
\cline{2-5}
& RU Agent & SE Agent & RU Agent & SE Agent  \\
\hline
10 & 0.18 &0.63 & 0.833& 1.09 \\ 
15$^*$ & 0.18 & 0.85 & 0.79&2.30 \\
20 & 0.13 &0.66 & 0.63 & 1.92 \\
25 & 0.42 & 0.55 & 0.00 & 2.00 \\
\hline
\end{tabular}
 \caption{\label{tab:scene_generator_results} Performance of the Scene Exploration Agent}
\end{table}

together table
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{Num. Nodes} & \multicolumn{2}{c|}{Objects Hidden} & %
    \multicolumn{2}{c|}{Stability Index} & \multicolumn{2}{c|}{Fraction of scenes solved} & %
    \multicolumn{2}{c|}{Objects found}\\
\cline{2-9}
%  & \multicolumn{2}{c|}{Value} & \multicolumn{2}{c|}{Value} & \\
% \cline{2-5}
 & RU Agent & SG Agent & RU Agent & SG Agent & RU Agent & SE Agent & RU Agent & SE Agent\\
\hline
10 & 0.94 & \textbf{2.09} & 0.84 & \textbf{0.99} & 0.18 &0.63 & 0.833& 1.09 \\
% 11 & 0.9559 & \textbf{2.3655} & 0.79 & \textbf{0.95} \\
% 12 & 0.904 & \textbf{2.3618} & 0.8 & \textbf{0.98} \\
% 13 & 1.1544 & \textbf{2.2795} & 0.78 & \textbf{0.97} \\
% 14 & 0.9792 & \textbf{2.328} & 0.64 & \textbf{0.97} \\
15$^*$ & 1.04 & \textbf{2.38} & 0.64 & \textbf{0.99} & 0.18 & 0.85 & 0.79&2.30 \\
% 16 & 1.0595 & \textbf{2.3232} & 0.65 & \textbf{0.96} \\
% 17 & 1.2474 & \textbf{2.2932} & 0.63 & \textbf{0.98} \\
% 18 & 1.27968 & \textbf{2.2736} & 0.62 & \textbf{0.98} \\
% 19 & 1.0556 & \textbf{2.1945} & 0.52 & \textbf{0.95} \\
20 & 1.19 & \textbf{2.28} & 0.55 & \textbf{0.93} & 0.13 &0.66 & 0.63 & 1.92 \\
25 & 1.02 & \textbf{2.43} & 0.41 & \textbf{0.81} & 0.42 & 0.55 & 0.00 & 2.00 \\
\hline
% \label{tab:scene_generator_results}
\end{tabular}
 \caption{\label{tab:scene_generator_results} Performance of the Scene Generator Agent (SG) compared to Random Uniform Agent (RU). Stability index is the fraction of simulated scenes that end up being physically stable.}
\end{table}

==> real_robot_discussion.tex <==
\section{Discussion about Real Robot Experiments}
The goal of our work is to design robotic agents that can interactively explore cluttered scenes of objects that have an underlying structure. However, due to the social distancing guidelines put in place due to Covid-19 and limited access to robotic hardware, we were unable to test out our approach on a real robot. Therefore, we have taken multiple steps to ensure that our approach can be transferred to real hardware (sim2real) by ensuring that the learned networks are robust to variations in scene structure and manipulation errors:
\emph{(i)} We perturb objects that the agent rearranges in the scene, by imparting a small velocity ($7$cm/s in our experiments) along a random direction on the XY-plane, to simulate real world actuator error and ensure stability of the scene despite such errors;
\emph{(ii)} Our Scene Generation Agent is trained using maximum entropy RL to generate a distribution of difficult and stable scene graphs. While these scene graphs define the underlying structure of the scene, we add an additional element of randomness in generated scenes by randomly sampling the location of each object that is placed on the tray. This further adds to the diversity in initial state distribution of the Scene Exploration Agent;
\emph{(iii)} Our approach is also independent of the exact type of manipulator used as long it can perform pick-and-place style manipulations and we show examples of such manipulations using a UR10 robot attached with a Robotiq e-pick end-effector in simulation;
\emph{(iv)} We also have a realistic perception pipeline that uses a state-of-the-art CNN based object detector. 
Since this module can be trained independent of our RL pipeline, we can use any pre-trained object detector and eliminate the need for excessive real world data collection and annotation. 

While our method reliably scales across a diverse set of scenes and is robust to simulated actuation errors, we hope to conduct experiments on a real-world setup. We anticipate that we could gain additional insight on how other physical attributes of a scene, such as lighting and shadows, could be leveraged to inform interactive exploration. 
To test our method in the real world we intend to use a pre-trained object detector and a 6D pose detection network as the robot's perception system. 
We can transfer our exploration network trained in simulation, directly to the real world by feeding it the partial scene graphs generated from the real robot's perception system. 
Since our exploration method is already exposed to a diverse distribution of cluttered scene arrangements and can generalize to different graph sizes, we expect to achieve successful sim2real transfer.
